Deep Learning Closure of the Navier-Stokes Equations for Transition-Continuum Flows

The predictive accuracy of the Navier-Stokes equations is known to degrade at the limits of the continuum assumption, thereby necessitating expensive and often highly approximate solutions to the Boltzmann equation. While tractable in one spatial dimension, their high dimensionality makes multi-dimensional Boltzmann calculations impractical for all but canonical configurations. It is therefore desirable to augment the Navier-Stokes equations in these regimes. We present an application of a deep learning method to extend the validity of the Navier-Stokes equations to the transition-continuum flows. The technique encodes the missing physics via a neural network, which is trained directly from Boltzmann solutions. While standard DL methods can be considered ad-hoc due to the absence of underlying physical laws, at least in the sense that the systems are not governed by known partial differential equations, the DL framework leverages the a-priori known Boltzmann physics while ensuring that the trained model is consistent with the Navier-Stokes equations. The online training procedure solves adjoint equations, constructed using algorithmic differentiation, which efficiently provide the gradient of the loss function with respect to the learnable parameters. The model is trained and applied to predict stationary, one-dimensional shock thickness in low-pressure argon.

==> macrtl-macros.tex <==
\usepackage{xcolor}
\usepackage{tikz}
\usepackage{stackrel}
\usepackage{bm,bbm}% bold math
\usepackage[version=3]{mhchem}

\usepackage{multirow}
\usepackage{setspace}
\usepackage{yfonts}
\usepackage{mathrsfs}
\usepackage{tcolorbox}
\usepackage{colortbl}
\usepackage{commath}
\usepackage{multicol}

% Support for Pandoc-beamer
\usepackage[T1]{fontenc}
\usepackage{booktabs}
\usepackage{longtable}
\usepackage{fancyvrb}
\providecommand{\tightlist}{%
  \setlength{\itemsep}{0pt}\setlength{\parskip}{0pt}}

\usepackage[retainorgcmds]{IEEEtrantools}
\usepackage{siunitx}     
\sisetup{detect-display-math=true,detect-weight=true,detect-family=true}

\usepackage{tcolorbox,xcolor,framed}
\DefineVerbatimEnvironment{Highlighting}{Verbatim}{fontsize=\footnotesize,commandchars=\\\{\}}
\definecolor{shadecolor}{rgb}{0.9,0.9,0.9}
\newenvironment{Shaded}{\snugshade}{\endsnugshade}
\newcommand{\KeywordTok}[1]{\textcolor[rgb]{0.13,0.29,0.53}{\textbf{#1}}}
\newcommand{\DataTypeTok}[1]{\textcolor[rgb]{0.13,0.29,0.53}{#1}}
\newcommand{\NormalTok}[1]{#1}
\newcommand{\DecValTok}[1]{\textcolor[rgb]{0.00,0.00,0.81}{#1}}
\newcommand{\CommentTok}[1]{\textcolor[rgb]{0.56,0.35,0.01}{\textit{{#1}}}}
\newcommand{\PreprocessorTok}[1]{\textcolor[rgb]{0.56,0.35,0.01}{\textit{{#1}}}}
\newcommand{\ControlFlowTok}[1]{\textcolor[rgb]{0.13,0.29,0.53}{\textbf{{#1}}}}


\usepackage[colorinlistoftodos, color=blue!20!white, bordercolor=gray,
textsize=tiny]{todonotes}


\makeatletter
\newcommand*{\overlaynumber}{\number\beamer@slideinframe}
\makeatother

\usepackage{pgf}
\usetikzlibrary{arrows,shapes,shapes.arrows,positioning,calc,decorations.text}

\usepackage{standalone}



\usepackage{multimedia}
\usepackage{graphicx}
\usepackage{animate}
%\usepackage{minted}

\definecolor{pdcolor1}{RGB}{23,35,57}    % ND blue  (Formal Palette)
\definecolor{pdcolor2}{RGB}{184,152,80}  % ND gold  (Formal Palette)
%\definecolor{pdcolor2}{RGB}{150,123,61}  % ND gold  (Formal Palette)
\definecolor{pdcolor3}{RGB}{60,132,62}  % ND green (Formal Palette)





\def \d {\mathrm{d}}
\def \dd#1#2{\frac{\mathrm{d} #1}{\mathrm{d} #2}}
\def \pp#1#2{\frac{\partial #1}{\partial #2}}
\newcommand{\dprime}[1]{^{\prime\prime #1}}
\newcommand{\sprime}[1]{^{\prime #1}}
\newcommand{\ol}[1]{\overline{#1}}
\newcommand{\wt}[1]{\widetilde{#1}}
\newcommand{\oll}[1]{\overline{#1}_\lambda}
\newcommand{\wtl}[1]{\widetilde{#1}_\lambda}
\newcommand{\RE}{{Re}}
\newcommand{\Da}{{Da}}
\newcommand{\Ka}{{Ka}}
\def \rhom {\overline{\rho}}
%\newcommand{\Pl}{P(\lambda)}
\newcommand{\Pl}{\widetilde{P}}

\def\Put(#1,#2)#3{\leavevmode\makebox(0,0){\put(#1,#2){#3}}}
\newcommand{\mynote}[1]{{\color{green} \tiny #1}}
\newcommand{\prj}[2]{{\color{gray} #1 [#2]}}
\newcommand{\noprj}[2]{}
\newcommand{\talkref}[2]{{\color{gray} #1 [#2]}}
\newcommand{\makered}[1]{{\color{red} #1}}
\newcommand{\makeblue}[1]{{\color{blue} #1}}
\newcommand{\makegreen}[1]{{\color{green} #1}}
\newcommand{\maketeal}[1]{{\color{teal} #1}}
\newcommand{\makeorange}[1]{{\color{orange} #1}}

\newcommand{\clink}{{\tiny({\color{blue} link})}}


\newcommand{\myoul}[1]{\color{pdcolor2}\underline{\smash{\color{pdcolor1} #1}}\color{pdcolor1}}
\newcommand{\ccdot}{\color{pdcolor2}$\circ$\color{pdcolor1}\;}
\newcommand{\cc}[1]{\color{pdcolor2}#1\color{pdcolor1}{}}

\newcommand{\HRule}[2]{{\color{pdcolor2}\rule{#1}{#2}}}
\newcommand{\dRightarrow}{{\color{pdcolor2}\Rightarrow}}
\newcommand{\dLeftarrow}{{\color{pdcolor2}\Leftarrow}}
\newcommand{\tb}[1]{{\color{blue}(#1)}}
\newcommand{\tr}[1]{{\color{blue}({\color{red}#1})}}
\newcommand{\tor}[1]{{\color{blue}({\color{blue}#1})}}
\newcommand{\lead}[1]{\textit{\color{pdcolor2}(#1)}}
\newcommand{\bmath}{\boldsymbol}
\newcommand{\eps}{\varepsilon}
\newcommand{\vp}{\vec{p}}
\newcommand{\rPI}[1]{{\color{pdcolor2}#1}}
\newcommand{\gPI}[1]{{\color{pdcolor3}#1}}
\newcommand{\tPI}[1]{\texttt{\color{pdcolor2}#1}}
\newcommand{\ttPI}[1]{\texttt{\color{pdcolor2}#1}}
\newcommand{\cPI}[1]{\textbf{\color{pdcolor2}#1}}
\newcommand{\iPI}[1]{\textit{\color{pdcolor2}#1}}
\newcommand{\sPI}[1]{\textsc{\color{pdcolor2}#1}}
\newcommand{\scPI}[1]{\textsc{\color{pdcolor2}#1}}
\newcommand{\tabtit}[1]{\textsc{\color{pdcolor2}#1}}
\newcommand{\Dpartial}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\bU}{\mathbf{U}}
\newcommand{\obsigma}{{\bar \sigma}}
\newcommand{\vsigma}{\vec{\sigma}}
\newcommand{\II}{{I\!I}}
\newcommand{\memph}[1]{{\color{red} #1}}
\newcommand{\eg}{\emph{e.g.}}
\newcommand{\mat}[1]{\ensuremath{\mathsf{#1}}}
\newcommand{\bvec}[1]{\ensuremath{\boldsymbol{#1}}}



\newcommand{\sectionWithFrame}[1]{%
  \section{#1}
  \begin{frame}
    \centerline{\LARGE \insertsection}
  \end{frame}}
\newcommand{\sectionAndsubWithFrame}[2]{%
  \section{#1}
  \begin{frame}
    \centerline{\LARGE \insertsection}
    \bigskip
    \centerline{\large #2}
  \end{frame}}

\newcommand{\cM}{\mathcal{M}}
\newcommand{\cT}{\mathcal{T}}

\newcommand{\bn}{\mathbf{n}}

\newcommand{\bbC}{\mathbb{C}}
\newcommand{\vbbm}{{\vec{m}}}
\newcommand{\bbM}{\mathbb{M}}
\newcommand{\bbH}{\mathbb{H}}
\newcommand{\bbG}{\mathbb{G}}
\newcommand{\bbV}{\mathbb{V}}

\newcommand{\vD}{{\vec D}}
\newcommand{\vhD}{{\hat{D}}}
\newcommand{\vg}{{\vec g}}
\newcommand{\vphi}{{\vec\phi}}
\newcommand{\vOmega}{{\vec\Omega}}

\newcommand{\vF}{{\vec{F}}}
\newcommand{\vf}{{\vec{f}}}
\newcommand{\vb}{{\vec{b}}}
\newcommand{\vq}{{\vec{q}}}
\newcommand{\vqs}{{\vec{q}^{\,\color{red}*}}}

\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cQ}{\mathcal{Q}}

\newcommand{\rstar}{{\color{red}*}}
\newcommand{\rchk}{{\color{red} \checkmark}}
\newcommand{\rex}{{\color{red} \xmark}}
\newcommand{\gchk}{{\color{green} \checkmark}}
\newcommand{\rbul}{{\color{red} $\bullet$}}
\newcommand{\pbul}{{\color{pdcolor2} $\bullet$}}
\newcommand{\ro}{{\color{red} $\circ$}}
\newcommand{\bd}{{\color{blue} $\bullet$}}

\newcommand{\rhoi}[1][i]{\rho_{#1}}
\newcommand{\dt}[1][t]{\partial_{#1}}
\newcommand{\dx}[1][{\textrm{\bf x}}]{\boldsymbol \partial_{#1}}
\newcommand{\Vi}[1][i]{\mathcal{V}_{#1}}
\newcommand{\Mi}[1][\textswab{i}]{\mathcal{M}_{#1}}
\newcommand{\omegai}[1][i]{\dot{\omega}_{#1}}
\newcommand{\grav}{{\bf g}}
\newcommand{\Etot}{\mathcal{E}}

\newcommand{\mBG}{m_{\text{\tiny BG}}}
\newcommand{\nBG}{n_{\text{\tiny BG}}}
\newcommand{\nIp}{n_{\text{\tiny $I^+$}}}
\newcommand{\nIm}{n_{\text{\tiny $I^-$}}}


\newcommand{\bI}{{\mathbf{I}}}
\newcommand{\bq}{{\mathbf{q}}}
\newcommand{\btau}{{\boldsymbol{\tau}}}

\newcommand{\bv}{{\bar{v}}}
\newcommand{\bepsilon}{{\bar{\epsilon}}}

\newcommand{\ST}{{S_{\text{\tiny T}}}}

\newcommand{\vu}{\vec{u}}
\newcommand{\vQ}{\vec{Q}}
\newcommand{\veta}{\vec{\eta}}


  \newcommand{\Grad}{\bnabla}
  \newcommand{\Div}{\bnabla\vdot}
  \newcommand{\Curl}{\bnabla\vprod}
  \newcommand{\hGrad}{\bnabla^{}_{\!\!\mathrm{h}}}
  \newcommand{\hDiv}{\bnabla^{}_{\!\!\mathrm{h}}\!\vdot}
  \newcommand{\pGrad}{\bnabla^{}_{\!\!\!\perp}}
  \newcommand{\pDiv}{\bnabla^{}_{\!\!\!\perp}\!\vdot}
\newcommand{\pop}[2]{\frac{\partial #1}{\partial #2}}
%\newcommand{\pp}[1]{\ensuremath{\left[ #1 \right]}}
\newcommand{\psq}[1]{\ensuremath{{\left[ #1 \right]}}}

% Grad, div, curl, etc.
\newcommand{\vdot}{\mathop{\mbox{\boldmath{$\cdot$}}}}
\newcommand{\vddot}{\mathop{\mbox{\textbf{:}}}}
\newcommand{\bnabla}{\mbox{\boldmath{$\nabla$}}}
\newcommand{\Lapl}{\nabla^2}
\newcommand{\hLapl}{\nabla^2_{\!\mathrm{h}}}
\newcommand{\pLapl}{\nabla^2_{\!\!\!\perp}}

\newcommand{\kION}{k_{\text{\tiny ION}}}
\newcommand{\kDET}{k_{\text{\tiny DET}}}
\newcommand{\kDR}{k_{\text{\tiny DR}}}
\newcommand{\kDA}{k_{\text{\tiny DA}}}
\newcommand{\kII}{k_{\text{\tiny $II$}}}


\def\colorize<#1>{%
\temporal<#1>{}{\color{red}}{}
}

\newcommand{\TODO}[1]{{\color{red} \tiny TODO: #1}}
\newcommand{\CHK}{{\color{red} ???}}
\newcommand{\CHKWDG}{{\color{red} ???WDG???}}
\newcommand{\progname}[1]{\textit{#1}}
\newcommand{\PlasComCM}{\progname{PlasComCM}}
\newcommand{\PlasComCMtwo}{\progname{PlasCom2}}
\newcommand{\plascomtwo}{\progname{PlasCom2}}
\newcommand{\dancode}{\PlasComCM}
\newcommand{\dancodetwo}{\progname{PlasCom2}}
\newcommand{\codelet}[1]{\progname{Codelet-#1}}
\newcommand{\goldenCopy}{\rPI{golden copy}}
\newcommand{\GoldenCopy}{\rPI{Golden copy}}
\newcommand{\code}[1]{\texttt{#1}}
\newcommand{\PCtwo}{\progname{PlasCom2}}
\newcommand{\CSTUF}{\progname{CSTUF}}

\newcommand{\xnew}{$^{\text{\tiny \makered{new}}}$}
\newcommand{\xremind}{$^{\text{\tiny \makeblue{reminder}}}$}
\newcommand{\Q}[1]{{\medskip\small\noindent\color{red}#1\par}}

\newcommand{\insertmovie}[3]{\ifmovies{
\movie[autostart,loop]
{\includegraphics[width=#1\textwidth]{Movies/#2}}
{Movies/#3}
}
\else{
\includegraphics[width=#1\textwidth]{Movies/#2}
}
\fi
}



\definecolor{ForestGreen}{rgb}{0.0, 0.2, 0.13}
\definecolor{darkpastelgreen}{rgb}{0.01, 0.75, 0.24}
\definecolor{antiquewhite}{rgb}{0.98, 0.92, 0.84}

\newcommand{\planA}{$\mathbb{A}$}
\newcommand{\planAA}{$\mathcal{A}'$}
\newcommand{\planB}{B}

\newcommand{\MUST}{{\footnotesize\color{red} \textbf{MUST}}}
\newcommand{\WISH}{{\footnotesize\color{orange} \textbf{WISH}}}
\newcommand{\DEFER}{{\footnotesize\color{yellow} \textbf{DEFER}}}
\newcommand{\WDEFER}{{\footnotesize\color{lightgray} \textbf{DEFER}}}
\newcommand{\RETURN}{{\footnotesize\color{blue} \textbf{RETURN}}}
\newcommand{\DONE}{{\footnotesize\color{ForestGreen} \textbf{COMPLETED}}}
\newcommand{\PLAN}{{\footnotesize\color{green} \textbf{PLANNED}}}
\newcommand{\CURRENT}{{\footnotesize\color{cyan} \textbf{NOW}}}

\newcommand{\SNL}{{\footnotesize $\;\rightarrow$ SNL}}
\newcommand{\LLNL}{{\footnotesize $\;\rightarrow$ LLNL}}
\newcommand{\LANL}{{\footnotesize $\;\rightarrow$ LANL}}


\newcommand{\aMUST}{\tiny\raisebox{1.5pt}{\color{red} (\textbf{M})}}
\newcommand{\aWISH}{\raisebox{1.5pt}{\tiny\color{orange} (\textbf{W})}}
\newcommand{\aDEFER}{\raisebox{1.5pt}{\tiny\color{yellow} (\textbf{D})}}
\newcommand{\aRETURN}{\raisebox{1.5pt}{\tiny\color{blue} (\textbf{R})}}
\newcommand{\aDONE}{\raisebox{1.5pt}{\tiny\color{ForestGreen} (\textbf{C})}}
\newcommand{\aPLAN}{\raisebox{1.5pt}{\tiny\color{green} (\textbf{P})}}
\newcommand{\aCURRENT}{\raisebox{1.5pt}{\tiny\color{cyan} (\textbf{N})}}

\newcommand{\Resp}{\cPI{Planned Response}}
\newcommand{\Recm}{\cPI{Recommendation}}

\newcommand{\gdotfill}{{\color{gray}\dotfill}}

\newcommand{\recbox}[1]{
\fcolorbox{pdcolor2}{antiquewhite}{
\begin{minipage}{0.97\textwidth}
\noindent
\Recm:
{#1}
\end{minipage}}
}
\newcommand{\recb}[1]{\fcolorbox{pdcolor2}{antiquewhite}{\Recm: #1}}

\newcommand{\recboxnt}[1]{
\fcolorbox{pdcolor2}{antiquewhite}{
\begin{minipage}{0.97\textwidth}
{#1}
\end{minipage}}
}

\arrayrulecolor{pdcolor2}

\usepackage{pgfplots}
\usepackage{pgfplotstable}

\definecolor{RYB1}{RGB}{207, 37, 37}
\definecolor{RYB2}{RGB}{37, 91, 207}
\definecolor{RYB3}{RGB}{37, 207, 91}
\definecolor{RYB4}{RGB}{163,26,145}
\definecolor{RYB5}{RGB}{253, 180, 98}
\definecolor{RYB6}{RGB}{179, 222, 105}
\definecolor{RYB7}{RGB}{128, 177, 211}

\pgfplotscreateplotcyclelist{newcolors}{
{RYB1,every mark/.append style={fill=RYB1,mark size={2.5}},mark=*},
{RYB2,every mark/.append style={fill=RYB2},mark=square*},
{RYB3,every mark/.append style={fill=RYB3,mark size={3}},mark=triangle*},
{RYB4,every mark/.append style={fill=RYB4,mark size={4}},mark=x},
{RYB5,every mark/.append style={fill=RYB5,mark size={3}},mark=oplus},
%{RYB6,every mark/.append style={fill=RYB6,mark size={4}},mark=10-pointed star},
{RYB7,every mark/.append style={fill=RYB7},mark=*},
}
\pgfplotsset{
  %  every axis/.append style={
 %       scale only axis,
 %      width=0.5\textwidth,
%    },
    standard/.style={
    thick,
    compat=1.8,
            scale only axis,
        width=0.45\textwidth,
  %      axis x line=middle,
%        axis y line=middle,
        enlarge x limits=0.05,
        enlarge y limits=0.05,
  %      every axis x label/.style={at={(current axis.right of origin)},anchor=north west},
  %      every axis y label/.style={at={(current axis.above origin)},anchor=north east},
        max space between ticks=40,
 %       tick label style={font=\Large},
%label style={font=\Large},
%legend style={font=\Large},
cycle list name=newcolors
%    cycle list={RYB1\\RYB2\\RYB3\\RYB4\\RYB5}
    }
}

